Generic non-trivial resonances for Anosov diffeomorphisms

We study real analytic perturbations of hyperbolic linear automorphisms on the 2-torus. The Koopman and the transfer operator are nuclear of order 0 when acting on a suitable Hilbert space. We show the generic existence of non-trivial Ruelle resonances for both operators. We prove that some of the perturbations preserve the volume and some of them do not.

==> preliminaries.tex <==
\section{Preliminaries}\label{s:PREL}
%\subsection{Notation}
Throughout this work we denote\ftBranch{}{ for every $d\in\MB{N}$} the flat \ftBranch{$2$}{$d$}-torus by \ftBranch{$\MB{T}^2\dfn \MB{R}^2/\MB{Z}^2$}{$\MB{T}^d\dfn \MB{R}^d/\MB{Z}^d$}. We embed $\VS{\MB{T}}$ into the standard polyannulus in $\VS{\MB{C}}$ and set for each $r>0$ \[\STRIP{r}\dfn \VS{\MB{T}}+\iunit\VS{\mb{-r,r}}\ft{.}\]
We see $\STRIP{r}$ as a submanifold of $\VS{\MB{C}}$.
% and tangent space is identified with \[T\MB{A}_{r,d}\cong \MB{R}^d+\iunit\MB{R}^d\ft{.}\]
%For every differentiable map $T\colon\MB{T}^d\rightarrow\MB{T}^d$, we denote by $\DIFF{T}\colon\MB{R}^d\rightarrow\MB{R}^d$ the derivative of $T$ at $x\in\MB{T}^d$.
% We use the ${}^*$ to indicate the corresponding element of the dual space or the adjoint operator.
% In particular, we use the realization $\mb{\VS{\MB{R}}}^*\cong\VS{\MB{R}}$. Analogously the transposed of a linear map $M\colon \VS{\MB{R}}\rightarrow \VS{\MB{R}}$ is denoted by $M^*$.
%\subsection{Spaces of dynamics and perturbations}
%The latter set $\MC{B}_{d,r}$ is just a Banach space which lies dense in the Hilbert space $H^2\mb{\MB{A}_{r,d}}$ known as a generalization of the Hardy space to an polyannulus \cite{boyd_composition_1976}.
%\ftBranch{We}{For $d\in\MB{N}$ we} say that a map $T\colon\VS{\MB{T}}\rightarrow\VS{\MB{T}}$ has for some $r>0$ a holomorphic extension to a polyannulus $\STRIP{r}$ if there is a lift $\tilde{T}\colon\MB{R}^d\rightarrow\MB{R}^d$ of $T$ which has a holomorphic extension to $\MB{R}^d+\iunit\mb{-r,r}^d$ and satisfies the $1$-coboundary condition
%\[\tilde{T}\mb{x+n}-\tilde{T}\mb{x}\in\MB{Z}^d\ft{,}\quad\forall n\in\MB{Z}^d\ft{, }x\in\MB{R}^d\ft{.}\]
%Whenever possible we identify $T$ with $\tilde{T}$.
%As an example consider the expanding map \[\tilde{T}\colon\MB{R}\rightarrow\MB{R}\colon x\mapsto 2x\ft{.}\]
%This non-periodic real analytic map descends to a non-injective map $T$ on $\MB{T}$ having a non-vanishing derivative everywhere and two surjective branches. In general $T$ has always finitely many everywhere differentiable branches because of real analyticity. Without any further restrictions on $T$ such branches may not be surjective, e.g. consider the map $\frac{1}{4}\sin\mb{2\pi x}$, $x\in\MB{R}$.
We set
\[\PERT[\MC{T}]\dfn\mbs{T\colon\TORUS\rightarrow\TORUS\SR T\ft{ extends holomorphically and bounded on }\STRIP{r}}\ft{.}\]
For every $\mb{\ftBranch{z_1,z_2}{z_1,\dots,z_d}}^{\trp}\in \VS{\MB{C}}$ and $p\in\mbs{1,2}$ we let $\mnp[p]{z}\dfn\mb{\ftBranch{\mbm{z_1}^p+\mbm{z_2}^p}{\sum_{n=1}^d\mbm{z_n}^p}}^{\frac 1p}$. We say that two maps $f$, $g\in\PERT[\MC{T}]$ are $C^1$-close if the function
\[\mnp[2]{f-g}+\sup_{z\in\STRIP{r}}{\mnp[2]{\mb{\DIFF[]f-\DIFF[]g}z}}\]
is small on $\STRIP{r}$.   
%This is a normed $\MB{Z}$-module and the submodule having a $\MB{Z}^d$-periodic lift is a Banach space yielding the perturbations of the dynamics in the $C^1$-topology.
%For each $T\in\MC{P}_{d,r}$ we set
%\[\mnp[\infty]{T}\dfn \sup_{z\in\STRIP[r,d]}\mbm{T\mb{z}}\ft{.}\]
%Endowed with this norm the completion of $\MC{P}_{d,r}$ becomes a Banach space denoted by $\MC{B}_{d,r}\ft{.}$
%%Since $\MC{B}_{d,r}$ contains all the Fourier polynomials \wrt $\MC{H}_{d,r}$ it is a dense set in $\MC{H}_{d,r}$.
%Note that $\MC{T}_{d,r}$ contains e.g. all linear maps contrary to $\MC{B}_{d,r}$ while being only a $\MB{Z}$-module.
